A Primal-Dual Partial Inverse Splitting for Constrained Monotone Inclusions: Applications to stochastic Programming and Mean Field Games

In this work we study a constrained monotone inclusion involving the normal cone to a closed vector subspace and a priori information on primal solutions. We model this information by imposing that solutions belongs to the fixed point set of an averaged nonexpansive mapping. We characterize the solutions using an auxiliary inclusion that involves the partial inverse operator. Then, we propose the primal-dual partial inverse splitting and we prove its weak convergence to a solution of the inclusion, generalizing several methods in the literature. The efficiency of the proposed method is illustrated in two non-smooth convex optimization problems whose constraints have vector subspace structure. Finally, the proposed algorithm is applied to find a solution to a stochastic arc capacity expansion problem in transport networks.

==> references.tex <==
@book {1,
    AUTHOR = {Bauschke, Heinz H. and Combettes, Patrick L.},
     TITLE = {Convex Analysis and Monotone Operator Theory in 
     {H}ilbert
              Spaces},
    SERIES = {CMS Books in Mathematics/Ouvrages de Math\'{e}matiques de la SMC},
   EDITION = {Second},
 PUBLISHER = {Springer},
      YEAR = {2017},
      ISBN = {978-3-319-48310-8; 978-3-319-48311-5},
   MRCLASS = {49-02 (41A65 46B20 46C05 47H05 90C25)},
  MRNUMBER = {3616647},
ADDRESS={Cham},
       DOI = {10.1007/978-3-319-48311-5},
}

@article{Vanden20b,
  title={Bregman primal--dual first-order method and application to 
  sparse semidefinite programming},
  author={Jiang, Xin and Vandenberghe, Lieven},
  year={2021},
  note={http://www.seas.ucla.edu/~vandenbe/publications/sdp-bregman.pdf},
}


@article {Micc11,
    AUTHOR = {Micchelli, Charles A. and Shen, Lixin and Xu, 
    Yuesheng},
     TITLE = {Proximity algorithms for image models: denoising},
   JOURNAL = {Inverse Problems},
  FJOURNAL = {Inverse Problems. An International Journal on the 
  Theory and
              Practice of Inverse Problems, Inverse Methods and 
              Computerized
              Inversion of Data},
    VOLUME = {27},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {045009, 30},
      ISSN = {0266-5611},
   MRCLASS = {94A08 (62H35 65D18 65J15 68U10)},
  MRNUMBER = {2781033},
MRREVIEWER = {R\'{e}mi Vaillancourt},
       DOI = {10.1088/0266-5611/27/4/045009},
}

@inproceedings{fadili09,
  title={Monotone operator splitting for optimization problems in sparse 
  recovery},
  author={Fadili, Mohamed-Jalal and Starck, J-L},
  booktitle={2009 16th IEEE International Conference on Image 
  Processing (ICIP)},
  pages={1461--1464},
  year={2009},
}

@INPROCEEDINGS{Cote17,
  author={Côté, François D. and Psaromiligkos, Ioannis N. and Gross, 
  Warren J.},
  booktitle={2017 IEEE Global Conference on Signal and Information 
  Processing (GlobalSIP)}, 
  title={A theory of generalized proximity for {ADMM}}, 
  year={2017},
  volume={},
  number={},
  pages={578-582},
  doi={10.1109/GlobalSIP.2017.8309025}}

@article {Vanden20,
    AUTHOR = {O'Connor, Daniel and Vandenberghe, Lieven},
     TITLE = {On the equivalence of the primal-dual hybrid gradient 
     method
              and {D}ouglas-{R}achford splitting},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {179},
      YEAR = {2020},
    NUMBER = {1-2, Ser. A},
     PAGES = {85--108},
      ISSN = {0025-5610},
   MRCLASS = {90C25 (47N10 49M27 49M29 65K05)},
  MRNUMBER = {4050138},
MRREVIEWER = {Hongjin He},
       DOI = {10.1007/s10107-018-1321-1},
}

@article{siopt3,
      title={{S}plit-{D}ouglas-{R}achford algorithm for composite 
      monotone 
      inclusions and {S}plit-{ADMM}}, 
      author={Luis M. Briceño-Arias and Fernando Roldán},
	  journal={SIAM J. Optim.},      
	  year={2021},
      note={to appear, https://arxiv.org/abs/2101.11683},
}

@misc{condat2020proximal,
      title={Proximal Splitting Algorithms: A Tour of Recent Advances, 
      with New Twists}, 
      author={Laurent Condat and Daichi Kitahara and Andrés 
      Contreras and Akira Hirabayashi},
      year={2020},
      eprint={1912.00137},
      archivePrefix={arXiv},
      primaryClass={math.OC},
note={https://arxiv.org/pdf/1912.00137.pdf},
}

@article {Comb_warped,
	AUTHOR = {B\`ui, Minh N. and Combettes, Patrick L.},
	TITLE = {Warped proximal iterations for monotone inclusions},
	JOURNAL = {J. Math. Anal. Appl.},
	FJOURNAL = {Journal of Mathematical Analysis and 
	Applications},
	VOLUME = {491},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {124315, 21},
	ISSN = {0022-247X},
	MRCLASS = {47J25 (47H05 47J22)},
	MRNUMBER = {4115560},
	MRREVIEWER = {Yu. V. Trubnikov},
	DOI = {10.1016/j.jmaa.2020.124315},
	URL = 
	{https://doi-org.usm.idm.oclc.org/10.1016/j.jmaa.2020.124315},
}

@article {Combvu14,
	AUTHOR = {Combettes, Patrick L. and V\~{u}, B\u{a}ng C.},
	TITLE = {Variable metric forward-backward splitting with 
	applications
	to monotone inclusions in duality},
	JOURNAL = {Optimization},
	FJOURNAL = {Optimization. A Journal of Mathematical 
	Programming and
	Operations Research},
	VOLUME = {63},
	YEAR = {2014},
	NUMBER = {9},
	PAGES = {1289--1318},
	ISSN = {0233-1934},
	MRCLASS = {47J25 (49M37 90C33 90C48)},
	MRNUMBER = {3225845},
	MRREVIEWER = {J. Borwein},
	DOI = {10.1080/02331934.2012.733883},
	URL = 
	{https://doi-org.usm.idm.oclc.org/10.1080/02331934.2012.733883},
}

@article {Moudafi14,
	AUTHOR = {Moudafi, Abdellatif},
	TITLE = {Computing the resolvent of composite operators},
	JOURNAL = {Cubo},
	FJOURNAL = {Cubo. A Mathematical Journal},
	VOLUME = {16},
	YEAR = {2014},
	NUMBER = {3},
	PAGES = {87--96},
	ISSN = {0716-7776},
	MRCLASS = {47J25 (65K10 90C25)},
	MRNUMBER = {3288323},
	DOI = {10.4067/s0719-06462014000300007},
	URL = 
	{https://doi-org.usm.idm.oclc.org/10.4067/s0719-06462014000300007},
}
@article {Fuku96,
	AUTHOR = {Fukushima, Masao},
	TITLE = {The primal {D}ouglas-{R}achford splitting algorithm for 
	a class of monotone mappings with application to the traffic
	equilibrium problem},
	JOURNAL = {Math. Programming},
	FJOURNAL = {Mathematical Programming},
	VOLUME = {72},
	YEAR = {1996},
	NUMBER = {1, Ser. A},
	PAGES = {1--15},
	ISSN = {0025-5610},
	MRCLASS = {90C33 (90C08)},
	MRNUMBER = {1385160},
	MRREVIEWER = {Bart De Schutter},
	DOI = {10.1016/0025-5610(95)00012-7},
	URL = 
	{https://doi-org.usm.idm.oclc.org/10.1016/0025-5610(95)00012-7},
}

@article {Giss_warped,
    AUTHOR = {Giselsson, Pontus},
     TITLE = {Nonlinear {F}orward-{B}ackward {S}plitting with 
     {P}rojection
              {C}orrection},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {31},
      YEAR = {2021},
    NUMBER = {3},
     PAGES = {2199--2226},
      ISSN = {1052-6234},
   MRCLASS = {49J40 (47 65K05 90C25 90C48)},
  MRNUMBER = {4308697},
       DOI = {10.1137/20M1345062},
}

@article {Moreau_cone,
    AUTHOR = {Moreau, Jean-Jacques},
     TITLE = {D\'{e}composition orthogonale d'un espace hilbertien 
     selon deux
              c\^{o}nes mutuellement polaires},
   JOURNAL = {C. R. Acad. Sci. Paris},
  FJOURNAL = {Comptes Rendus Hebdomadaires des S\'{e}ances de 
  l'Acad\'{e}mie des
              Sciences},
    VOLUME = {255},
      YEAR = {1962},
     PAGES = {238--240},
      ISSN = {0001-4036},
   MRCLASS = {46.15},
  MRNUMBER = {139919},
MRREVIEWER = {I. G. Amemiya},
}

@article {Moreau_prox,
    AUTHOR = {Moreau, Jean-Jacques},
     TITLE = {Proximit\'{e} et dualit\'{e} dans un espace hilbertien},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'{e}t\'{e} Math\'{e}matique de 
  France},
    VOLUME = {93},
      YEAR = {1965},
     PAGES = {273--299},
      ISSN = {0037-9484},
   MRCLASS = {46.15 (41.60)},
  MRNUMBER = {201952},
MRREVIEWER = {I. G. Amemiya},
}

@Article{Tang19,
	AUTHOR = {Yang, Yixuan and Tang, Yuchao and Zhu, 
	Chuanxi},
	TITLE = {Iterative Methods for Computing the Resolvent of 
	Composed Operators in {H}ilbert Spaces},
	JOURNAL = {Mathematics},
	VOLUME = {7},
	YEAR = {2019},
	NUMBER = {2},
	ARTICLE-NUMBER = {131},
	ISSN = {2227-7390},
	DOI = {10.3390/math7020131}
}

@article {Bot_grad,
	AUTHOR = {Bo\c{t}, Radu Ioan and Grad, Sorin-Mihai and 
	Wanka, Gert},
	TITLE = {Maximal monotonicity for the precomposition with a 
	linear
	operator},
	JOURNAL = {SIAM J. Optim.},
	FJOURNAL = {SIAM Journal on Optimization},
	VOLUME = {17},
	YEAR = {2006},
	NUMBER = {4},
	PAGES = {1239--1252},
	ISSN = {1052-6234},
	MRCLASS = {47H05 (47N10 90C25)},
	MRNUMBER = {2274512},
	MRREVIEWER = {Fumiaki Kohsaka},
	DOI = {10.1137/050641491},
}
@book {RieszNagy,
    AUTHOR = {Riesz, Frigyes and Sz.-Nagy, B\'{e}la},
     TITLE = {Functional analysis},
      NOTE = {Translated by Leo F. Boron},
 PUBLISHER = {Frederick Ungar Publishing Co., New York},
      YEAR = {1955},
     PAGES = {xii+468},
   MRCLASS = {46.2X},
  MRNUMBER = {0071727},
}

@article{vonMises,
author = {Mises, R. V. and Pollaczek-Geiringer, H.},
title = {Praktische Verfahren der Gleichungsauflösung .},
journal = {ZAMM - Journal of Applied Mathematics and Mechanics / 
Zeitschrift für Angewandte Mathematik und Mechanik},
volume = {9},
number = {2},
pages = {152-164},
doi = {10.1002/zamm.19290090206},
year = {1929}
} 

@article{gabaymercier,
author = {Daniel Gabay and Bertrand Mercier},
title = {A dual algorithm for the solution of nonlinear variational 
problems via finite element approximation},
journal = {Computers \& Mathematics with Applications},
volume = {2},
number = {1},
pages = {17-40},
year = {1976},
issn = {0898-1221},
doi = {10.1016/0898-1221(76)90003-1},
}

@article {shefi,
    AUTHOR = {Shefi, Ron and Teboulle, Marc},
     TITLE = {Rate of convergence analysis of decomposition methods 
     based on
              the proximal method of multipliers for convex minimization},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {24},
      YEAR = {2014},
    NUMBER = {1},
     PAGES = {269--297},
      ISSN = {1052-6234},
   MRCLASS = {90C25 (47J25)},
  MRNUMBER = {3166972},
MRREVIEWER = {Ern\"{o} Robert Csetnek},
       DOI = {10.1137/130910774},
}
@article {ap1,
    AUTHOR = {Attouch, H\'{e}dy and Brice\~{n}o-Arias, Luis M. and 
    Combettes,
              Patrick L.},
     TITLE = {A parallel splitting method for coupled monotone 
     inclusions},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {48},
      YEAR = {2009/10},
    NUMBER = {5},
     PAGES = {3246--3270},
      ISSN = {0363-0129},
   MRCLASS = {90C48 (47J25 49M30 90C25)},
  MRNUMBER = {2599918},
MRREVIEWER = {Michael Patriksson},
       DOI = {10.1137/090754297},
       URL = {https://doi-org.usm.idm.oclc.org/10.1137/090754297},
}
@article {Attouch,
    AUTHOR = {Attouch, H. and Soueycatt, M.},
     TITLE = {Augmented {L}agrangian and proximal alternating 
     direction
              methods of multipliers in {H}ilbert spaces. {A}pplications to
              games, {PDE}'s and control},
   JOURNAL = {Pac. J. Optim.},
  FJOURNAL = {Pacific Journal of Optimization. An International 
  Journal},
    VOLUME = {5},
      YEAR = {2009},
    NUMBER = {1},
     PAGES = {17--37},
      ISSN = {1348-9151},
   MRCLASS = {49J40 (47N10 49J20 49M30 91A10)},
  MRNUMBER = {2489926},
MRREVIEWER = {Jan Mach},
}

@article {BrediesSun15TV,
    AUTHOR = {Bredies, Kristian and Sun, Hong Peng},
     TITLE = {Preconditioned {D}ouglas-{R}achford algorithms for {TV}- 
     and
              {TGV}-regularized variational imaging problems},
   JOURNAL = {J. Math. Imaging Vision},
  FJOURNAL = {Journal of Mathematical Imaging and Vision},
    VOLUME = {52},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {317--344},
      ISSN = {0924-9907},
   MRCLASS = {94A08},
  MRNUMBER = {3345399},
       DOI = {10.1007/s10851-015-0564-1},
}

@article{Yang21,
title = {Preconditioned Douglas-Rachford type primal-dual method for 
solving composite monotone inclusion problems with applications},
journal = {Inverse Problems \& Imaging},
volume = {15},
number = {4},
pages = {787-825},
year = {2021},
author = {Yixuan Yang, Yuchao Tang, Meng Wen, Tieyong Zeng},
}

@article {BrediesSun15,
    AUTHOR = {Bredies, Kristian and Sun, Hongpeng},
     TITLE = {Preconditioned {D}ouglas-{R}achford splitting methods for
              convex-concave saddle-point problems},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {53},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {421--444},
      ISSN = {0036-1429},
   MRCLASS = {65K10 (49K35 65F08 90C25)},
  MRNUMBER = {3310980},
MRREVIEWER = {Jos\'{e} Eduardo Souza de Cursi},
       DOI = {10.1137/140965028},
}

@article {Osher11,
    AUTHOR = {Zhang, Xiaoqun and Burger, Martin and Osher, 
    Stanley},
     TITLE = {A unified primal-dual algorithm framework based on 
     {B}regman
              iteration},
   JOURNAL = {J. Sci. Comput.},
  FJOURNAL = {Journal of Scientific Computing},
    VOLUME = {46},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {20--46},
      ISSN = {0885-7474},
   MRCLASS = {90C25 (65D18 65F10 94A08)},
  MRNUMBER = {2753250},
MRREVIEWER = {Xiaojun Chen},
       DOI = {10.1007/s10915-010-9408-8},
}

@book {ReedSimon,
    AUTHOR = {Reed, Michael and Simon, Barry},
     TITLE = {Methods of modern mathematical physics. {I} Functional 
     analysis},
   EDITION = {Second},
 PUBLISHER = {Academic Press, Inc., New York},
      YEAR = {1980},
     PAGES = {xv+400},
      ISBN = {0-12-585050-6},
   MRCLASS = {46-01 (47-01)},
  MRNUMBER = {751959},
}

@article {BrediesSun17,
    AUTHOR = {Bredies, Kristian and Sun, Hongpeng},
     TITLE = {A proximal point analysis of the preconditioned alternating
              direction method of multipliers},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {173},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {878--907},
      ISSN = {0022-3239},
   MRCLASS = {65K10 (65F08 90C25)},
  MRNUMBER = {3654261},
MRREVIEWER = {Sirma Zeynep Alparslan-G\"{o}k},
       DOI = {10.1007/s10957-017-1112-5},
}

@article {CombVu14,
    AUTHOR = {Combettes, Patrick L. and V\~{u}, B\u{a}ng C.},
     TITLE = {Variable metric forward-backward splitting with 
     applications
              to monotone inclusions in duality},
   JOURNAL = {Optimization},
  FJOURNAL = {Optimization. A Journal of Mathematical 
  Programming and
              Operations Research},
    VOLUME = {63},
      YEAR = {2014},
    NUMBER = {9},
     PAGES = {1289--1318},
      ISSN = {0233-1934},
   MRCLASS = {47J25 (49M37 90C33 90C48)},
  MRNUMBER = {3225845},
MRREVIEWER = {J. Borwein},
       DOI = {10.1080/02331934.2012.733883},
}

@INPROCEEDINGS{pockcham,
  author={Pock, Thomas and Chambolle, Antonin},
  booktitle={2011 International Conference on Computer Vision}, 
  title={Diagonal preconditioning for first order primal-dual algorithms 
  in convex optimization}, 
  year={2011},
  volume={},
  number={},
  pages={1762-1769},
  doi={10.1109/ICCV.2011.6126441}}

@article {ChenTeb94,
    AUTHOR = {Chen, Gong and Teboulle, Marc},
     TITLE = {A proximal-based decomposition method for convex 
     minimization
              problems},
   JOURNAL = {Math. Programming},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {64},
      YEAR = {1994},
    NUMBER = {1, Ser. A},
     PAGES = {81--101},
      ISSN = {0025-5610},
   MRCLASS = {90C25},
  MRNUMBER = {1274173},
MRREVIEWER = {Khalil Mouallif},
       DOI = {10.1007/BF01582566},
}

@misc{BAR19,
	title={Primal-dual splittings as fixed point iterations in the range of 
	linear operators},
	author={{Brice\~no-Arias}, Luis M. and {Rold\'an}, F.},
	year={2019},
	eprint={1910.02329},
	archivePrefix={arXiv},
	primaryClass={math.OC}
}

@article {lions-mercier79,
	AUTHOR = {Lions, P.-L. and Mercier, B.},
	TITLE = {Splitting algorithms for the sum of two nonlinear operators},
	JOURNAL = {SIAM J. Numer. Anal.},
	FJOURNAL = {SIAM Journal on Numerical Analysis},
	VOLUME = {16},
	YEAR = {1979},
	NUMBER = {6},
	PAGES = {964--979},
	ISSN = {0036-1429},
	MRCLASS = {47H17 (35K55 35R35 49D25 65J15)},
	MRNUMBER = {551319},
	MRREVIEWER = {D. Pascali},
	DOI = {10.1137/0716071},
}

@article {Siopt2,
	AUTHOR = {{Brice\~{n}o-Arias}, Luis M. and Davis, Damek},
	TITLE = {Forward-backward-half forward algorithm for solving monotone
	inclusions},
	JOURNAL = {SIAM J. Optim.},
	FJOURNAL = {SIAM Journal on Optimization},
	VOLUME = {28},
	YEAR = {2018},
	NUMBER = {4},
	PAGES = {2839--2871},
	ISSN = {1052-6234},
	MRCLASS = {47J25 (47H05 65K05 65K15 90C25)},
	MRNUMBER = {3860903},
	MRREVIEWER = {Phan Tu Vuong},
	DOI = {10.1137/17M1120099},
}

@article {BausMoursi,
	AUTHOR = {Bauschke, Heinz H. and Moursi, Walaa M.},
	TITLE = {On the {D}ouglas-{R}achford algorithm},
	JOURNAL = {Math. Program.},
	FJOURNAL = {Mathematical Programming},
	VOLUME = {164},
	YEAR = {2017},
	NUMBER = {1-2, Ser. A},
	PAGES = {263--284},
	ISSN = {0025-5610},
	MRCLASS = {47H05 (47H09 47J25 49N15 90C25)},
	MRNUMBER = {3661032},
	MRREVIEWER = {Radu Ioan Bo\c{t}},
	DOI = {10.1007/s10107-016-1086-3},
}

@article {bauschetal2012,
	AUTHOR = {Bauschke, Heinz H. and Bo\c{t}, Radu I. and Hare, Warren L. and
	Moursi, Walaa M.},
	TITLE = {Attouch-{T}h\'{e}ra duality revisited: paramonotonicity and
	operator splitting},
	JOURNAL = {J. Approx. Theory},
	FJOURNAL = {Journal of Approximation Theory},
	VOLUME = {164},
	YEAR = {2012},
	NUMBER = {8},
	PAGES = {1065--1084},
	ISSN = {0021-9045},
	MRCLASS = {47H05 (41A50 49N15)},
	MRNUMBER = {2935445},
	MRREVIEWER = {Shoham Sabach},
	DOI = {10.1016/j.jat.2012.05.008},
}


@incollection {BauschkeFirmly,
    AUTHOR = {Bauschke, Heinz H.},
     TITLE = {New demiclosedness principles for (firmly) nonexpansive
              operators},
 BOOKTITLE = {Computational and analytical mathematics},
    SERIES = {Springer Proc. Math. Stat.},
    VOLUME = {50},
     PAGES = {19--28},
 PUBLISHER = {Springer, New York},
      YEAR = {2013},
   MRCLASS = {47H05 (47H09 47J25 49J53 65J15 90C25)},
  MRNUMBER = {3108420},
MRREVIEWER = {Patrick L. Combettes},
       DOI = {10.1007/978-1-4614-7621-4_2},
}
	
@article {BauschkeOrder,
    AUTHOR = {Bauschke, Heinz H. and Moursi, Walaa M.},
     TITLE = {On the order of the operators in the {D}ouglas-{R}achford
              algorithm},
   JOURNAL = {Optim. Lett.},
  FJOURNAL = {Optimization Letters},
    VOLUME = {10},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {447--455},
      ISSN = {1862-4472},
   MRCLASS = {47H09 (47H05 49M27 65K05 90C25)},
  MRNUMBER = {3463507},
MRREVIEWER = {Szil\'{a}rd Csaba L\'{a}szl\'{o}},
       DOI = {10.1007/s11590-015-0920-5},
}	

@INPROCEEDINGS{CPockDiag,
	author={T. {Pock} and A. {Chambolle}},
	booktitle={2011 International Conference on Computer Vision},
	title={Diagonal preconditioning for first order primal-dual algorithms in convex 
	optimization},
	year={2011},
	volume={},
	number={},
	pages={1762-1769},
	keywords={computer vision;convex programming;image denoising;linear 
	programming;diagonal preconditioning technique;first order primal-dual algorithm;convex 
	optimization;monotropic programming;linear programming;computer 
	vision;Convergence;IP networks;Symmetric matrices;Algorithm design and 
	analysis;Partitioning algorithms;Computer vision;Vectors},
	doi={10.1109/ICCV.2011.6126441},
	ISSN={2380-7504},
	month={Nov},}

@incollection {TV-chambolle,
	AUTHOR = {Chambolle, Antonin and Caselles, Vicent and Cremers, Daniel
	and Novaga, Matteo and Pock, Thomas},
	TITLE = {An introduction to total variation for image analysis},
	BOOKTITLE = {Theoretical Foundations and Numerical Methods for Sparse
	Recovery},
	SERIES = {Radon Ser. Comput. Appl. Math.},
	VOLUME = {9},
	PAGES = {263--340},
	PUBLISHER = {Walter de Gruyter, Berlin},
	YEAR = {2010},
	MRCLASS = {65D18 (26B30 68U10)},
	MRNUMBER = {2731599},
	DOI = {10.1515/9783110226157.263},
}

@article{Davisconvrate,
    AUTHOR = {Davis, Damek},
     TITLE = {Convergence rate analysis of primal-dual splitting schemes},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {25},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {1912--1943},
      ISSN = {1052-6234},
   MRCLASS = {65K15 (47H05 65K05 90C25)},
  MRNUMBER = {3402786},
MRREVIEWER = {Michael M. Dediu},
       DOI = {10.1137/151003076},
}

@Inbook{Latafat2018,
	author="Latafat, Puya
	and Patrinos, Panagiotis",
	editor="Giselsson, Pontus
	and Rantzer, Anders",
	title="Primal-Dual Proximal Algorithms for Structured Convex Optimization: A Unifying 
	Framework",
	bookTitle="Large-Scale and Distributed Optimization",
	year="2018",
	publisher="Springer International Publishing",
	address="Cham",
	pages="97--120",
	abstract="We present a simple primal-dual framework for solving structured convex 
	optimization problems involving the sum of a Lipschitz-differentiable function and two 
	nonsmooth proximable functions, one of which is composed with a linear mapping. The 
	framework is based on the recently proposed asymmetric forward-backward-adjoint 
	three-term splitting (AFBA); depending on the value of two parameters, (extensions of) 
	known algorithms as well as many new primal-dual schemes are obtained. This allows for a 
	unified analysis that, among other things, establishes linear convergence under four 
	different regularity assumptions for the cost functions. Most notably, linear convergence is 
	established for the class of problems with piecewise linear-quadratic cost functions.",
	isbn="978-3-319-97478-1",
	doi="10.1007/978-3-319-97478-1_5",
}

@Article{Bauschke2018,
	AUTHOR = {Bauschke, Heinz H. and Schaad, Jason and Wang, Xianfu},
     TITLE = {On {D}ouglas-{R}achford operators that fail to be proximal
              mappings},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {168},
      YEAR = {2018},
    NUMBER = {1-2, Ser. B},
     PAGES = {55--61},
      ISSN = {0025-5610},
   MRCLASS = {47H09 (47H05 90C25)},
  MRNUMBER = {3767740},
MRREVIEWER = {Matthew K. Tam},
       DOI = {10.1007/s10107-016-1076-5},
}

@Article{Bauschke2017,
	AUTHOR = {Bauschke, Heinz H. and Lukens, Brett and Moursi, Walaa M.},
     TITLE = {Affine nonexpansive operators, {A}ttouch-{T}h\'{e}ra duality and
              the {D}ouglas-{R}achford algorithm},
   JOURNAL = {Set-Valued Var. Anal.},
  FJOURNAL = {Set-Valued and Variational Analysis},
    VOLUME = {25},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {481--505},
      ISSN = {1877-0533},
   MRCLASS = {47H05 (47H09 49M27 49M29 49N15 90C25)},
  MRNUMBER = {3694874},
MRREVIEWER = {Minh N. Dao},
       DOI = {10.1007/s11228-016-0399-y},
}
	

@article {combvu,
	AUTHOR = {Combettes, Patrick L. and V\~{u}, B\brevgrv{a}ng C.},
	TITLE = {Variable metric quasi-{F}ej\'{e}r monotonicity},
	JOURNAL = {Nonlinear Anal.},
	FJOURNAL = {Nonlinear Analysis. Theory, Methods \& Applications. An
	International Multidisciplinary Journal},
	VOLUME = {78},
	YEAR = {2013},
	PAGES = {17--31},
	ISSN = {0362-546X},
	MRCLASS = {90C25 (47H09 65J05)},
	MRNUMBER = {2992983},
	MRREVIEWER = {Radu Ioan Bo\c{t}},
	DOI = {10.1016/j.na.2012.09.008},
}

@Article{eckstein-bertsekas,
  AUTHOR = {Eckstein, Jonathan and Bertsekas, Dimitri P.},
     TITLE = {On the {D}ouglas-{R}achford splitting method and the proximal
              point algorithm for maximal monotone operators},
   JOURNAL = {Math. Programming},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {55},
      YEAR = {1992},
    NUMBER = {3, Ser. A},
     PAGES = {293--318},
      ISSN = {0025-5610},
   MRCLASS = {90C25 (65K05)},
  MRNUMBER = {1168183},
MRREVIEWER = {F. Giannessi},
       DOI = {10.1007/BF01581204},
}


@Article{skew,
  AUTHOR = {{Brice\~{n}o-Arias}, Luis M. and Combettes, Patrick 
  L.},
     TITLE = {A monotone + skew splitting model for composite monotone
              inclusions in duality},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {21},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {1230--1250},
      ISSN = {1052-6234},
   MRCLASS = {47H05 (49J53 65K05 90C25 90C48)},
  MRNUMBER = {2854581},
MRREVIEWER = {Aris Daniilidis},
       DOI = {10.1137/10081602X},
}

@Article{11.vu,
  AUTHOR = {V\~{u}, B\brevgrv{a}ng C\^{o}ng},
     TITLE = {A splitting algorithm for dual monotone inclusions involving
              cocoercive operators},
   JOURNAL = {Adv. Comput. Math.},
  FJOURNAL = {Advances in Computational Mathematics},
    VOLUME = {38},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {667--681},
      ISSN = {1019-7168},
   MRCLASS = {47J25 (47H05 90C25)},
  MRNUMBER = {3037034},
       DOI = {10.1007/s10444-011-9254-8},
}

@Article{condat,
  AUTHOR = {Condat, Laurent},
     TITLE = {A primal-dual splitting method for convex optimization
              involving {L}ipschitzian, proximable and linear composite
              terms},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {158},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {460--479},
      ISSN = {0022-3239},
   MRCLASS = {90C25 (90C06 90C48)},
  MRNUMBER = {3084386},
MRREVIEWER = {C. Ilioi},
       DOI = {10.1007/s10957-012-0245-9},
}

@Article{cp,
  AUTHOR = {Chambolle, Antonin and Pock, Thomas},
     TITLE = {A first-order primal-dual algorithm for convex problems 
     with applications to imaging},
   JOURNAL = {J. Math. Imaging Vision},
  FJOURNAL = {Journal of Mathematical Imaging and Vision},
    VOLUME = {40},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {120--145},
      ISSN = {0924-9907},
   MRCLASS = {94A08 (68U10 90C25)},
  MRNUMBER = {2782122},
       DOI = {10.1007/s10851-010-0251-1},
}


@Article{yuan,
  AUTHOR = {He, Bingsheng and Yuan, Xiaoming},
     TITLE = {Convergence analysis of primal-dual algorithms for a
              saddle-point problem: from contraction perspective},
   JOURNAL = {SIAM J. Imaging Sci.},
  FJOURNAL = {SIAM Journal on Imaging Sciences},
    VOLUME = {5},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {119--149},
      ISSN = {1936-4954},
   MRCLASS = {90C47 (65K10 68U10)},
  MRNUMBER = {2902659},
       DOI = {10.1137/100814494},
}


@Article{opti04,
  AUTHOR = {Combettes, Patrick L.},
     TITLE = {Solving monotone inclusions via compositions of nonexpansive
              averaged operators},
   JOURNAL = {Optimization},
  FJOURNAL = {Optimization. A Journal of Mathematical Programming and
              Operations Research},
    VOLUME = {53},
      YEAR = {2004},
    NUMBER = {5-6},
     PAGES = {475--504},
      ISSN = {0233-1934},
   MRCLASS = {47H10 (47H05 47N20 54H25)},
  MRNUMBER = {2115266},
MRREVIEWER = {Alexander J. Zaslavski},
       DOI = {10.1080/02331930412331327157},
}


@Article{svaiter,
AUTHOR = {Svaiter, B. F.},
     TITLE = {On weak convergence of the {D}ouglas-{R}achford method},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {49},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {280--287},
      ISSN = {0363-0129},
   MRCLASS = {47J25 (49J53)},
  MRNUMBER = {2783211},
       DOI = {10.1137/100788100},       
}
	
@incollection {ipa,
	AUTHOR = {Combettes, Patrick L.},
	TITLE = {Quasi-{F}ej\'{e}rian analysis of some optimization algorithms},
	BOOKTITLE = {Inherently Parallel Algorithms in Feasibility and 
	Optimization
	and their Applications ({H}aifa, 2000)},
	SERIES = {Stud. Comput. Math.},
	VOLUME = {8},
	PAGES = {115--152},
	PUBLISHER = {North-Holland, Amsterdam},
	YEAR = {2001},
	MRCLASS = {90C25 (90C48 90C52)},
	MRNUMBER = {1853220},
	DOI = {10.1016/S1570-579X(01)80010-0},
}
@book{brezis,
  AUTHOR = {Brezis, Haim},
     TITLE = {Functional analysis, {S}obolev spaces and partial differential
              equations},
    SERIES = {Universitext},
 PUBLISHER = {Springer, New York},
      YEAR = {2011},
     PAGES = {xiv+599},
      ISBN = {978-0-387-70913-0},
   MRCLASS = {35-01 (46-01 46E35 46N20 47F05)},
  MRNUMBER = {2759829},
MRREVIEWER = {Vicen\c{t}iu D. R\u{a}dulescu},
}


@book{deblur,
  AUTHOR = {Hansen, Per Christian and Nagy, James G. and O'Leary, Dianne
              P.},
     TITLE = {Deblurring images: Matrices, spectra, and filtering},
    SERIES = {Fundamentals of Algorithms},
    VOLUME = {3},
 PUBLISHER = {Society for Industrial and Applied Mathematics (SIAM),
              Philadelphia, PA},
      YEAR = {2006},
     PAGES = {xiv+130},
      ISBN = {978-0-898716-18-4; 0-89871-618-7},
   MRCLASS = {94A08 (65D18 68U10)},
  MRNUMBER = {2271138},
       DOI = {10.1137/1.9780898718874},
}


@Article{peypou,
  author =	 { R. Cominetti and J. Peypouquet and S. Sorin },
  title = {Strong asymptotic convergence of evolution equations governed by maximal monotone operators with Tikhonov regularization},
  journal =	 {Journal of Differential Equations},
  doi =		 {10.1016/j.jde.2008.08.007},
  volume =	 245,
  number =	 12,
  year =	 2008,
  pages =	 {3753-3763},
}

@Article{FISTA,
  AUTHOR = {Beck, Amir and Teboulle, Marc},
     TITLE = {A fast iterative shrinkage-thresholding algorithm for linear
              inverse problems},
   JOURNAL = {SIAM J. Imaging Sci.},
  FJOURNAL = {SIAM Journal on Imaging Sciences},
    VOLUME = {2},
      YEAR = {2009},
    NUMBER = {1},
     PAGES = {183--202},
      ISSN = {1936-4954},
   MRCLASS = {35R30 (65F22 90C06 90C25)},
  MRNUMBER = {2486527},
       DOI = {10.1137/080716542},
}

@phdthesis{thesisNelly,
	TITLE = {{Proximal methods for the resolution of inverse problems : application to positron 
	emission tomography}},
	AUTHOR = {Pustelnik, Nelly},
	NUMBER = {2010PEST1037},
	SCHOOL = {{Universit{\'e} Paris-Est}},
	YEAR = {2010},
	MONTH = Dec,
	KEYWORDS = {Pet ; Wavelet frame ; Poisson noise ; Proximal algorithms ; Convex 
	optimization ; Inverse problems ; Probl{\`e}mes inverses ; Tep ; Trames d'ondelettes ; Bruit 
	de Poisson ; Algorithmes proximaux ; Optimisation convexe},
	TYPE = {Theses},
	PDF = {https://pastel.archives-ouvertes.fr/tel-00559126/file/main.pdf},
	HAL_ID = {tel-00559126},
	HAL_VERSION = {v5},
}

@Article{Molinari2019,
    AUTHOR = {Molinari, Cesare and Peypouquet, Juan and 
    Roldan, Fernando},
     TITLE = {Alternating forward-backward splitting for linearly
              constrained optimization problems},
   JOURNAL = {Optim. Lett.},
  FJOURNAL = {Optimization Letters},
    VOLUME = {14},
      YEAR = {2020},
    NUMBER = {5},
     PAGES = {1071--1088},
      ISSN = {1862-4472},
   MRCLASS = {90C25 (65K05 90C48)},
  MRNUMBER = {4114399},
       DOI = {10.1007/s11590-019-01388-y},}

@Article{ROF,
  AUTHOR = {Rudin, Leonid I. and Osher, Stanley and Fatemi, Emad},
     TITLE = {Nonlinear total variation based noise removal algorithms},
   JOURNAL = {Phys. D},
  FJOURNAL = {Physica D. Nonlinear Phenomena},
    VOLUME = {60},
      YEAR = {1992},
    NUMBER = {1-4},
     PAGES = {259--268},
      ISSN = {0167-2789},
   MRCLASS = {94A08 (65D18 68U10)},
  MRNUMBER = {3363401},
       DOI = {10.1016/0167-2789(92)90242-F},
}



@Article{bot2013,
  AUTHOR = {Bo\c{t}, Radu Ioan and Hendrich, Christopher},
     TITLE = {A {D}ouglas-{R}achford type primal-dual method for solving
              inclusions with mixtures of composite and parallel-sum type
              monotone operators},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {23},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {2541--2565},
      ISSN = {1052-6234},
   MRCLASS = {47J25 (47H05 90C25)},
  MRNUMBER = {3144800},
MRREVIEWER = {Francisco J. Arag\'{o}n Artacho},
       DOI = {10.1137/120901106},
}


@Article{FISTATV,
  AUTHOR = {Beck, Amir and Teboulle, Marc},
     TITLE = {Fast gradient-based algorithms for constrained total variation
              image denoising and deblurring problems},
   JOURNAL = {IEEE Trans. Image Process.},
  FJOURNAL = {IEEE Transactions on Image Processing},
    VOLUME = {18},
      YEAR = {2009},
    NUMBER = {11},
     PAGES = {2419--2434},
      ISSN = {1057-7149},
   MRCLASS = {94A08 (68U10 90C25)},
  MRNUMBER = {2722312},
       DOI = {10.1109/TIP.2009.2028250},
}

@Article{figueiredo,
  author =	 { M. A. T. Figueiredo and  R. D. Nowak and S, J. Wright},
  title = {Gradient Projection for Sparse Reconstruction: Application to Compressed Sensing and Other Inverse Problems},
  journal =	 {IEEE Journal of Selected Topics in Signal Processing},
  doi =		 {10.1109/jstsp.2007.910281},
  volume =	 1,
  number =	 4,
  year =	 2007,
  pages =	 {586-596},
}

@book{wavelet,
  AUTHOR = {Mallat, St\'{e}phane},
     TITLE = {A wavelet tour of signal processing: The sparse way},
   EDITION = {Third},
 PUBLISHER = {Elsevier/Academic Press, Amsterdam},
      YEAR = {2009},
     PAGES = {xxii+805},
      ISBN = {978-0-12-374370-1},
   MRCLASS = {94A12 (94-01 94-02)},
  MRNUMBER = {2479996},
}

@book {frazier,
    AUTHOR = {Frazier, Michael W.},
     TITLE = {An introduction to wavelets through linear algebra},
    SERIES = {Undergraduate Texts in Mathematics},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1999},
     PAGES = {xvi+501},
      ISBN = {0-387-98639-1},
   MRCLASS = {42C40},
  MRNUMBER = {1692229},
}


@article {Wajs,
    AUTHOR = {Combettes, Patrick L. and Wajs, Val\'{e}rie R.},
     TITLE = {Signal recovery by proximal forward-backward splitting},
   JOURNAL = {Multiscale Model. Simul.},
  FJOURNAL = {Multiscale Modeling \& Simulation. A SIAM Interdisciplinary
              Journal},
    VOLUME = {4},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {1168--1200},
      ISSN = {1540-3459},
   MRCLASS = {94A12 (90C25 94A08)},
  MRNUMBER = {2203849},
       DOI = {10.1137/050626090},
       }

@article{lasso1,
    AUTHOR = {Tibshirani, Robert},
     TITLE = {Regression shrinkage and selection via the lasso},
   JOURNAL = {J. Roy. Statist. Soc. Ser. B},
  FJOURNAL = {Journal of the Royal Statistical Society. Series B.
              Methodological},
    VOLUME = {58},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {267--288},
      ISSN = {0035-9246},
   MRCLASS = {62J05 (62J07)},
  MRNUMBER = {1379242},
}

@article {lasso2,
    AUTHOR = {Zhao, Peng and Yu, Bin},
     TITLE = {On model selection consistency of {L}asso},
   JOURNAL = {J. Mach. Learn. Res.},
  FJOURNAL = {Journal of Machine Learning Research (JMLR)},
    VOLUME = {7},
      YEAR = {2006},
     PAGES = {2541--2563},
      ISSN = {1532-4435},
   MRCLASS = {62C05 (62J10)},
  MRNUMBER = {2274449},
}

@article {lasso3,
    AUTHOR = {Meinshausen, Nicolai and Yu, Bin},
     TITLE = {Lasso-type recovery of sparse representations for
              high-dimensional data},
   JOURNAL = {Ann. Statist.},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {37},
      YEAR = {2009},
    NUMBER = {1},
     PAGES = {246--270},
      ISSN = {0090-5364},
   MRCLASS = {62J07 (62F07 62J05)},
  MRNUMBER = {2488351},
       DOI = {10.1214/07-AOS582},
      }


	
	
@article {bauschkeDR,
    AUTHOR = {Bauschke, Heinz H. and Moursi, Walaa M.},
     TITLE = {On the {D}ouglas-{R}achford algorithm},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {164},
      YEAR = {2017},
    NUMBER = {1-2, Ser. A},
     PAGES = {263--284},
      ISSN = {0025-5610},
   MRCLASS = {47H05 (47H09 47J25 49N15 90C25)},
  MRNUMBER = {3661032},
MRREVIEWER = {Radu Ioan Bo\c{t}},
       DOI = {10.1007/s10107-016-1086-3},
      }

@INPROCEEDINGS{patrinos_opV,
author={P. {Sopasakis} and A. {Themelis} and J. {Suykens} and P. {Patrinos}},
booktitle={2017 25th European Signal Processing Conference (EUSIPCO)},
title={A primal-dual line search method and applications in image processing},
year={2017},
volume={},
number={},
pages={1065-1069},
keywords={image denoising;search problems;primal-dual line search method;image processing;operator splitting algorithms;Chambolle-Pock algorithm;SuperMann;image denoising;anisotropic total variation regularization;Signal processing algorithms;1/f noise;Convergence;Europe;Optimization;Search methods},
doi={10.23919/EUSIPCO.2017.8081371},
ISSN={2076-1465},
month={Aug},}





@article{BOT2,
AUTHOR = {Bo\c{t}, Radu Ioan and Csetnek, Ern\"{o} Robert and Heinrich, Andr\'{e}},
     TITLE = {A primal-dual splitting algorithm for finding zeros of sums of
              maximal monotone operators},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {23},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {2011--2036},
      ISSN = {1052-6234},
   MRCLASS = {47J25 (47H05 49J52 49N15 90C25)},
  MRNUMBER = {3116476},
MRREVIEWER = {Massimo Lanza de Cristoforis},
       DOI = {10.1137/12088255X},
}
	
@article {OP2015BA,
    AUTHOR = {{Brice\~{n}o-Arias}, Luis M.},
     TITLE = {Forward-{D}ouglas-{R}achford splitting and forward-partial
              inverse method for solving monotone inclusions},
   JOURNAL = {Optimization},
  FJOURNAL = {Optimization. A Journal of Mathematical Programming and
              Operations Research},
    VOLUME = {64},
      YEAR = {2015},
    NUMBER = {5},
     PAGES = {1239--1261},
      ISSN = {0233-1934},
   MRCLASS = {47H05 (47J25 65K05 90C25)},
  MRNUMBER = {3316800},
       DOI = {10.1080/02331934.2013.855210},
}
	


@article {J2015BA,
    AUTHOR = {{Brice\~{n}o-Arias}, Luis M.},
     TITLE = {Forward-partial inverse-forward splitting for solving monotone
              inclusions},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {166},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {391--413},
      ISSN = {0022-3239},
   MRCLASS = {47H05 (47J25 65J15 90C25)},
  MRNUMBER = {3371381},
MRREVIEWER = {Shenghua Wang},
       DOI = {10.1007/s10957-015-0703-2},
}

@article {tseng2000,
    AUTHOR = {Tseng, Paul},
     TITLE = {A modified forward-backward splitting method for maximal
              monotone mappings},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {38},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {431--446},
      ISSN = {0363-0129},
   MRCLASS = {49M27 (47H05 47J25 65J20)},
  MRNUMBER = {1741147},
MRREVIEWER = {Bernard Lemaire},
       DOI = {10.1137/S0363012998338806},
}


@article {Combettes2009resolventDR,
    AUTHOR = {Combettes, Patrick L.},
     TITLE = {Iterative construction of the resolvent of a sum of maximal
              monotone operators},
   JOURNAL = {J. Convex Anal.},
  FJOURNAL = {Journal of Convex Analysis},
    VOLUME = {16},
      YEAR = {2009},
    NUMBER = {3-4},
     PAGES = {727--748},
      ISSN = {0944-6532},
   MRCLASS = {49M29 (47H05 47J25 65K05 90C25)},
  MRNUMBER = {2583892},
MRREVIEWER = {Heinz H. Bauschke},
}

@article {spingarninverse,
    AUTHOR = {Spingarn, Jonathan E.},
     TITLE = {Partial inverse of a monotone operator},
   JOURNAL = {Appl. Math. Optim.},
  FJOURNAL = {Applied Mathematics and Optimization},
    VOLUME = {10},
      YEAR = {1983},
    NUMBER = {3},
     PAGES = {247--265},
      ISSN = {0095-4616},
   MRCLASS = {47H05 (49D39 65J15 90C33 90C48)},
  MRNUMBER = {722489},
MRREVIEWER = {B. T. Polyak},
       DOI = {10.1007/BF01448388},
}
	
	
	
@article {proximalforcontrol,
    AUTHOR = {Azhmyakov, Vadim and Morales, Salvador Noriega},
     TITLE = {Proximal point method for optimal control processes governed
              by ordinary differential equations},
   JOURNAL = {Asian J. Control},
  FJOURNAL = {Asian Journal of Control},
    VOLUME = {12},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {15--25},
      ISSN = {1561-8625},
   MRCLASS = {49M37 (49M25)},
  MRNUMBER = {2676767},
MRREVIEWER = {Olga Vasilieva},
       DOI = {10.1002/asjc.154},
}
		
@article {frederic1986,
    AUTHOR = {Bonnans, Joseph Fr\'{e}d\'{e}ric},
     TITLE = {On an algorithm for optimal control using {P}ontryagin's
              maximum principle},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {24},
      YEAR = {1986},
    NUMBER = {3},
     PAGES = {579--588},
      ISSN = {0363-0129},
   MRCLASS = {49D07},
  MRNUMBER = {838058},
MRREVIEWER = {Asen L. Dontchev},
       DOI = {10.1137/0324034},
}
		

@article {rockafellar1976,
    AUTHOR = {Rockafellar, R. Tyrrell},
     TITLE = {Monotone operators and the proximal point algorithm},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {14},
      YEAR = {1976},
    NUMBER = {5},
     PAGES = {877--898},
      ISSN = {0363-0129},
   MRCLASS = {47H05 (49D45)},
  MRNUMBER = {410483},
MRREVIEWER = {G. M. Ewing},
       DOI = {10.1137/0314056},
}				
	


@article {martinet1970,
        author = {Martinet, B.},
     title = {Br\`eve communication. R\'egularisation d'in\'equations variationnelles par approximations successives},
     journal = {ESAIM: Mathematical Modelling and Numerical Analysis - Mod\'elisation Math\'ematique et Analyse Num\'erique},
     publisher = {Dunod},
     volume = {4},
     number = {R3},
     year = {1970},
     pages = {154-158},
     zbl = {0215.21103},
     mrnumber = {298899},
     language = {fr},
}

@article {DR1956,
    AUTHOR = {Douglas, Jr., Jim and Rachford, Jr., H. H.},
     TITLE = {On the numerical solution of heat conduction problems in two
              and three space variables},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {82},
      YEAR = {1956},
     PAGES = {421--439},
      ISSN = {0002-9947},
   MRCLASS = {65.3X},
  MRNUMBER = {84194},
MRREVIEWER = {Charles Saltzer},
       DOI = {10.2307/1993056},
}
@article {Passty1979,
    AUTHOR = {Passty, Gregory B.},
     TITLE = {Ergodic convergence to a zero of the sum of monotone operators
              in {H}ilbert space},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {72},
      YEAR = {1979},
    NUMBER = {2},
     PAGES = {383--390},
      ISSN = {0022-247X},
   MRCLASS = {47H05 (49A29)},
  MRNUMBER = {559375},
MRREVIEWER = {R. A. Plastock},
       DOI = {10.1016/0022-247X(79)90234-8},
}		
	

	
@article {Goldstein64,
    AUTHOR = {Goldstein, A. A.},
     TITLE = {Convex programming in {H}ilbert space},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {70},
      YEAR = {1964},
     PAGES = {709--710},
      ISSN = {0002-9904},
   MRCLASS = {90.60},
  MRNUMBER = {165982},
MRREVIEWER = {A. V. Balakrishnan},
       DOI = {10.1090/S0002-9904-1964-11178-2},
}

@article {Tseng1991_variational,
    AUTHOR = {Tseng, Paul},
     TITLE = {Applications of a splitting algorithm to decomposition in
              convex programming and variational inequalities},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {29},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {119--138},
      ISSN = {0363-0129},
   MRCLASS = {90C25 (47H19 49J40 65K05)},
  MRNUMBER = {1088222},
MRREVIEWER = {Stephan Dempe},
       DOI = {10.1137/0329006},
}

@article {Tseng1990_variational,
    AUTHOR = {Tseng, Paul},
     TITLE = {Further applications of a splitting algorithm to decomposition
              in variational inequalities and convex programming},
   JOURNAL = {Math. Programming},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {48},
      YEAR = {1990},
    NUMBER = {2, (Ser. B)},
     PAGES = {249--263},
      ISSN = {0025-5610},
   MRCLASS = {90C25 (49J40)},
  MRNUMBER = {1073710},
MRREVIEWER = {Robert W. Owens},
       DOI = {10.1007/BF01582258},
}



@book {Mercier1980,
    AUTHOR = {Mercier, B.},
     TITLE = {In\'{e}quations variationnelles de la m\'{e}canique},
    SERIES = {Publications Math\'{e}matiques d'Orsay 80 [Mathematical
              Publications of Orsay 80]},
    VOLUME = {1},
 PUBLISHER = {Universit\'{e} de Paris-Sud, D\'{e}partement de Math\'{e}matique, Orsay},
      YEAR = {1980},
     PAGES = {98},
   MRCLASS = {49A29 (35Q20 65P05 73E05)},
  MRNUMBER = {570823},
MRREVIEWER = {N. Gass},
}
	@book {Zeidler1990,
    AUTHOR = {Zeidler, Eberhard},
     TITLE = {Nonlinear functional analysis and its applications. {II}/{B}},
      NOTE = {Nonlinear monotone operators,
              Translated from the German by the author and Leo F. Boron},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1990},
     PAGES = {i--xvi and 469--1202},
      ISBN = {0-387-97167-X},
   MRCLASS = {47-02 (35-01 35J60 47Hxx 58-01 65Jxx)},
  MRNUMBER = {1033498},
MRREVIEWER = {Jean Mawhin},
       DOI = {10.1007/978-1-4612-0985-0},
}


@article {Lions1967,
    AUTHOR = {Lions, J.-L. and Stampacchia, G.},
     TITLE = {Variational inequalities},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {20},
      YEAR = {1967},
     PAGES = {493--519},
      ISSN = {0010-3640},
   MRCLASS = {47.90 (35.00)},
  MRNUMBER = {216344},
MRREVIEWER = {T. R. Jenkins},
       DOI = {10.1002/cpa.3160200302},
}

@article {Jofre2007,
    AUTHOR = {Jofr\'{e}, Alejandro and Rockafellar, R. Terry and Wets, Roger
              J.-B.},
     TITLE = {Variational inequalities and economic equilibrium},
   JOURNAL = {Math. Oper. Res.},
  FJOURNAL = {Mathematics of Operations Research},
    VOLUME = {32},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {32--50},
      ISSN = {0364-765X},
   MRCLASS = {91B50 (49J40 90C47)},
  MRNUMBER = {2292496},
MRREVIEWER = {Vincenzo Scalzo},
       DOI = {10.1287/moor.1060.0233},
}
		
		@article {Pennanen2012,
    AUTHOR = {Pennanen, Teemu},
     TITLE = {Introduction to convex optimization in financial markets},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {134},
      YEAR = {2012},
    NUMBER = {1, Ser. B},
     PAGES = {157--186},
      ISSN = {0025-5610},
   MRCLASS = {91G80 (90C25)},
  MRNUMBER = {2947556},
       DOI = {10.1007/s10107-012-0573-4},
}
@article {Chambolle2005,
    AUTHOR = {Aujol, Jean-Fran\c{c}ois and Aubert, Gilles and Blanc-F\'{e}raud,
              Laure and Chambolle, Antonin},
     TITLE = {Image decomposition into a bounded variation component and an
              oscillating component},
   JOURNAL = {J. Math. Imaging Vision},
  FJOURNAL = {Journal of Mathematical Imaging and Vision},
    VOLUME = {22},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {71--88},
      ISSN = {0924-9907},
   MRCLASS = {68U10},
  MRNUMBER = {2138585},
       DOI = {10.1007/s10851-005-4783-8},
}

@article {Chambolle1997,
    AUTHOR = {Chambolle, Antonin and Lions, Pierre-Louis},
     TITLE = {Image recovery via total variation minimization and related
              problems},
   JOURNAL = {Numer. Math.},
  FJOURNAL = {Numerische Mathematik},
    VOLUME = {76},
      YEAR = {1997},
    NUMBER = {2},
     PAGES = {167--188},
      ISSN = {0029-599X},
   MRCLASS = {65K10 (49J99 68U10)},
  MRNUMBER = {1440119},
MRREVIEWER = {Tom\'{a}\v{s} Roub\'{\i}\v{c}ek},
       DOI = {10.1007/s002110050258},
}

@article {Daubechies2004,
    AUTHOR = {Daubechies, Ingrid and Defrise, Michel and De Mol, Christine},
     TITLE = {An iterative thresholding algorithm for linear inverse
              problems with a sparsity constraint},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {57},
      YEAR = {2004},
    NUMBER = {11},
     PAGES = {1413--1457},
      ISSN = {0010-3640},
   MRCLASS = {65J22 (35R30 47A52 65J20 65R30 90C30)},
  MRNUMBER = {2077704},
MRREVIEWER = {Hans-Peter Helfrich},
       DOI = {10.1002/cpa.20042},
}

@book {Aubin1990,
    AUTHOR = {Aubin, Jean-Pierre and Frankowska, H\'{e}l\`ene},
     TITLE = {Set-valued analysis},
    SERIES = {Systems \& Control: Foundations \& Applications},
    VOLUME = {2},
 PUBLISHER = {Birkh\"{a}user Boston, Inc., Boston, MA},
      YEAR = {1990},
     PAGES = {xx+461},
      ISBN = {0-8176-3478-9},
   MRCLASS = {49-02 (26-02 28-02 46-02 47H15 49J52 58C06 90C48)},
  MRNUMBER = {1048347},
MRREVIEWER = {Leszek Zaremba},
}

@book {Showalter1997,
    AUTHOR = {Showalter, R. E.},
     TITLE = {Monotone operators in {B}anach space and nonlinear partial
              differential equations},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {49},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {1997},
     PAGES = {xiv+278},
      ISBN = {0-8218-0500-2},
   MRCLASS = {47H15 (34G20 35J60 35K55 47H05 47N20)},
  MRNUMBER = {1422252},
MRREVIEWER = {Ioan I. Vrabie},
}

@article {Bertsekas1982,
    AUTHOR = {Bertsekas, Dimitri P. and Gafni, Eli M.},
     TITLE = {Projection methods for variational inequalities with
              application to the traffic assignment problem},
   JOURNAL = {Math. Programming Stud.},
  FJOURNAL = {Mathematical Programming Study},
    NUMBER = {17},
      YEAR = {1982},
     PAGES = {139--159},
      ISSN = {0303-3929},
   MRCLASS = {49A29 (65K10 90B20)},
  MRNUMBER = {654697},
MRREVIEWER = {Phan V\u{a}n Chuong},
       DOI = {10.1007/bfb0120965},
}

@article {Gilpin2012,
    AUTHOR = {Gilpin, Andrew and Pe\~{n}a, Javier and Sandholm, Tuomas},
     TITLE = {First-order algorithm with {$O(\ln(1/\epsilon))$} convergence for {$\epsilon$}-equilibrium in two-person zero-sum games},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {133},
      YEAR = {2012},
    NUMBER = {1-2, Ser. A},
     PAGES = {279--298},
      ISSN = {0025-5610},
   MRCLASS = {91A05 (90C47 90C52)},
  MRNUMBER = {2921100},
       DOI = {10.1007/s10107-010-0430-2},
}


@incollection{gabay83,
title = "Chapter {IX} Applications of the Method of Multipliers to 
Variational Inequalities",
editor = "Michel Fortin and Roland Glowinski",
series = "Studies in Mathematics and Its Applications",
publisher = "Elsevier",
volume = "15",
pages = "299 - 331",
year = "1983",
booktitle = "Augmented Lagrangian Methods: Applications to the Numerical Solution of Boundary-Value Problems",
issn = "0168-2024",
doi = "10.1016/S0168-2024(08)70034-1",
author = "D. Gabay",
address="New York",

}

@article {ecksteinadmm2015,
    AUTHOR = {Eckstein, Jonathan and Yao, Wang},
     TITLE = {Understanding the convergence of the alternating direction
              method of multipliers: theoretical and computational
              perspectives},
   JOURNAL = {Pac. J. Optim.},
  FJOURNAL = {Pacific Journal of Optimization. An International Journal},
    VOLUME = {11},
      YEAR = {2015},
    NUMBER = {4},
     PAGES = {619--644},
      ISSN = {1348-9151},
   MRCLASS = {90C25 (49M37 90C06)},
  MRNUMBER = {3420805},
MRREVIEWER = {Wim van Ackooij},
}

@article {salzo2017,
    AUTHOR = {Salzo, Saverio},
     TITLE = {The variable metric forward-backward splitting algorithm under
              mild differentiability assumptions},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {27},
      YEAR = {2017},
    NUMBER = {4},
     PAGES = {2153--2181},
      ISSN = {1052-6234},
   MRCLASS = {90C25 (65K05)},
  MRNUMBER = {3707899},
MRREVIEWER = {Juan Peypouquet},
       DOI = {10.1137/16M1073741},
}

@incollection {yin2016,
    AUTHOR = {Yan, Ming and Yin, Wotao},
     TITLE = {Self equivalence of the alternating direction method of
              multipliers},
 BOOKTITLE = {Splitting Methods in Communication, Imaging, 
 Science, and
              Engineering},
    SERIES = {Sci. Comput.},
     PAGES = {165--194},
 PUBLISHER = {Springer, Cham},
      YEAR = {2016},
   MRCLASS = {90C25},
  MRNUMBER = {3617563},
}
	
	
@article {bot2018,
    AUTHOR = {Bo\c{t}, Radu Ioan and Csetnek, Ern\"{o} Robert},
     TITLE = {A{DMM} for monotone operators: convergence analysis and rates},
   JOURNAL = {Adv. Comput. Math.},
  FJOURNAL = {Advances in Computational Mathematics},
    VOLUME = {45},
      YEAR = {2019},
    NUMBER = {1},
     PAGES = {327--359},
      ISSN = {1019-7168},
   MRCLASS = {47J25 (47H05 65K05 90C25 90C48)},
  MRNUMBER = {3915012},
MRREVIEWER = {Xiaolong Qin},
       DOI = {10.1007/s10444-018-9619-3},
}

@article {patrinos2020,
    AUTHOR = {Themelis, Andreas and Patrinos, Panagiotis},
     TITLE = {Douglas-{R}achford splitting and {ADMM} for nonconvex
              optimization: tight convergence results},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {30},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {149--181},
      ISSN = {1052-6234},
   MRCLASS = {90C26 (49J52 49J53 90C06 90C25)},
  MRNUMBER = {4049404},
MRREVIEWER = {Philippe Mahey},
       DOI = {10.1137/18M1163993},
}


@article {russell2016,
    AUTHOR = {Aspelmeier, Timo and Charitha, C. and Luke, D. Russell},
     TITLE = {Local linear convergence of the {ADMM}/{D}ouglas-{R}achford
              algorithms without strong convexity and application to
              statistical imaging},
   JOURNAL = {SIAM J. Imaging Sci.},
  FJOURNAL = {SIAM Journal on Imaging Sciences},
    VOLUME = {9},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {842--868},
   MRCLASS = {47J25 (47J15 49J52 49M20 65K05 90C26 94A08)},
  MRNUMBER = {3516863},
MRREVIEWER = {Nicolas Hadjisavvas},
       DOI = {10.1137/15M103580X},
}


@incollection {moursi2019,
    AUTHOR = {Moursi, Walaa M. and Zinchenko, Yuriy},
     TITLE = {A note on the equivalence of operator splitting methods},
 BOOKTITLE = {Splitting Algorithms, Modern Operator Theory, and
              Applications},
     PAGES = {331--349},
 PUBLISHER = {Springer, Cham},
      YEAR = {2019},
   MRCLASS = {47H05 (49M27 49M29 49N15 90C25 90C48)},
  MRNUMBER = {3971979},
}

@book {Showalter,
	AUTHOR = {Showalter, R. E.},
	TITLE = {Monotone Operators in {B}anach Space and 
	Nonlinear Partial
	Differential Equations},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {49},
	PUBLISHER = {American Mathematical Society, Providence, 
	RI},
	YEAR = {1997},
	PAGES = {xiv+278},
	ISBN = {0-8218-0500-2},
	MRCLASS = {47H15 (34G20 35J60 35K55 47H05 47N20)},
	MRNUMBER = {1422252},
	MRREVIEWER = {Ioan I. Vrabie},
	DOI = {10.1090/surv/049},
}
@article {Vu15,
    AUTHOR = {D\~{u}ng, Dinh and V\~{u}, B\brevgrv{a}ng 
    C\^{o}ng},
     TITLE = {A splitting algorithm for system of composite 
     monotone inclusions},
   JOURNAL = {Vietnam J. Math.},
  FJOURNAL = {Vietnam Journal of Mathematics},
    VOLUME = {43},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {323--341},
      ISSN = {2305-221X},
   MRCLASS = {47J25 (47H05 49M27 90C25)},
  MRNUMBER = {3349819},
       DOI = {10.1007/s10013-015-0121-7},
}

@article {EckSvaiter,
    AUTHOR = {Eckstein, Jonathan and Svaiter, B. F.},
     TITLE = {A family of projective splitting methods for the sum of 
     two maximal monotone operators},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming. A Publication of the 
  Mathematical
              Programming Society},
    VOLUME = {111},
      YEAR = {2008},
    NUMBER = {1-2, Ser. B},
     PAGES = {173--199},
      ISSN = {0025-5610},
   MRCLASS = {47H05 (47J25 47N10 49M27 90C25)},
  MRNUMBER = {2322888},
MRREVIEWER = {Radu Ioan Bo\c{t}},
       DOI = {10.1007/s10107-006-0070-8},
      }

@incollection {Nash,
	AUTHOR = {Brice\~{n}o-Arias, Luis M. and Combettes, Patrick 
	L.},
	TITLE = {Monotone operator methods for {N}ash equilibria in
	non-potential games},
	BOOKTITLE = {Computational and analytical mathematics},
	SERIES = {Springer Proc. Math. Stat.},
	VOLUME = {50},
	PAGES = {143--159},
	PUBLISHER = {Springer, New York},
	YEAR = {2013},
	MRCLASS = {91A05 (47H05 49J40 90C25)},
	MRNUMBER = {3108427},
	DOI = {10.1007/978-1-4614-7621-4_9},
}

@incollection {Bauschke2015,
    AUTHOR = {Bauschke, Heinz H. and Koch, Valentin R.},
     TITLE = {Projection methods: {S}wiss army knives for solving
              feasibility and best approximation problems with halfspaces},
 BOOKTITLE = {Infinite Products of Operators and their 
 Applications},
    SERIES = {Contemp. Math.},
    VOLUME = {636},
     PAGES = {1--40},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2015},
   MRCLASS = {65K05 (41A29 49M37 90C25)},
  MRNUMBER = {3155358},
MRREVIEWER = {Etienne de Klerk},
       DOI = {10.1090/conm/636/12726},
}

@article {Fuku96,
	AUTHOR = {Fukushima, Masao},
	TITLE = {The primal {D}ouglas-{R}achford splitting algorithm for 
	a
	class of monotone mappings with application to the traffic
	equilibrium problem},
	JOURNAL = {Math. Programming},
	FJOURNAL = {Mathematical Programming},
	VOLUME = {72},
	YEAR = {1996},
	NUMBER = {1, Ser. A},
	PAGES = {1--15},
	ISSN = {0025-5610},
	MRCLASS = {90C33 (90C08)},
	MRNUMBER = {1385160},
	MRREVIEWER = {Bart De Schutter},
	DOI = {10.1016/0025-5610(95)00012-7},
}

@article {ChambLions97,
	AUTHOR = {Chambolle, Antonin and Lions, Pierre-Louis},
	TITLE = {Image recovery via total variation minimization and 
	related
	problems},
	JOURNAL = {Numer. Math.},
	FJOURNAL = {Numerische Mathematik},
	VOLUME = {76},
	YEAR = {1997},
	NUMBER = {2},
	PAGES = {167--188},
	ISSN = {0029-599X},
	MRCLASS = {65K10 (49J99 68U10)},
	MRNUMBER = {1440119},
	MRREVIEWER = {Tom\'{a}\v{s} Roub\'{\i}\v{c}ek},
	DOI = {10.1007/s002110050258},
}


@article {Nets1,
	AUTHOR = {Brice\~{n}o, Luis and Cominetti, Roberto and 
	Cort\'{e}s, Cristi\'{a}n E.
	and Mart\'{\i}nez, Francisco},
	TITLE = {An integrated behavioral model of land use and 
	transport
	system: a hyper-network equilibrium approach},
	JOURNAL = {Netw. Spat. Econ.},
	FJOURNAL = {Networks and Spatial Economics},
	VOLUME = {8},
	YEAR = {2008},
	NUMBER = {2-3},
	PAGES = {201--224},
	ISSN = {1566-113X},
	MRCLASS = {91D10 (90B10)},
	MRNUMBER = {2410998},
	DOI = {10.1007/s11067-007-9052-5},
}

@article {GafniBert84,
	AUTHOR = {Gafni, Eli M. and Bertsekas, Dimitri P.},
	TITLE = {Two-metric projection methods for constrained 
	optimization},
	JOURNAL = {SIAM J. Control Optim.},
	FJOURNAL = {SIAM Journal on Control and Optimization},
	VOLUME = {22},
	YEAR = {1984},
	NUMBER = {6},
	PAGES = {936--964},
	ISSN = {0363-0129},
	MRCLASS = {90C30 (65K10)},
	MRNUMBER = {762631},
	MRREVIEWER = {Jon W. Tolle},
	DOI = {10.1137/0322061},
}

@article {Daube04,
	AUTHOR = {Daubechies, Ingrid and Defrise, Michel and De 
	Mol, Christine},
	TITLE = {An iterative thresholding algorithm for linear inverse
	problems with a sparsity constraint},
	JOURNAL = {Comm. Pure Appl. Math.},
	FJOURNAL = {Communications on Pure and Applied 
	Mathematics},
	VOLUME = {57},
	YEAR = {2004},
	NUMBER = {11},
	PAGES = {1413--1457},
	ISSN = {0010-3640},
	MRCLASS = {65J22 (35R30 47A52 65J20 65R30 90C30)},
	MRNUMBER = {2077704},
	MRREVIEWER = {Hans-Peter Helfrich},
	DOI = {10.1002/cpa.20042},
}


@article{Boyd2011,
year = {2011},
volume = {3},
journal = {Foundations and Trends in Machine Learning},
title = {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
doi = {10.1561/2200000016},
issn = {1935-8237},
number = {1},
pages = {1-122},
author = {Stephen Boyd and Neal Parikh and Eric Chu and Borja Peleato and Jonathan Eckstein}
}

@phdthesis{ecksteinthesis,
  title={Splitting Methods for Monotone Operators with 
  Applications to Parallel Optimization},
  author={Eckstein, Jonathan},
  year={1989},
  school={Massachusetts Institute of Technology}
}


@article {GlowinskyMorrocco75,
    AUTHOR = {Glowinski, R. and Marrocco, A.},
     TITLE = {Sur l'approximation, par \'{e}l\'{e}ments finis d'ordre un, et la
              r\'{e}solution, par p\'{e}nalisation-dualit\'{e}, d'une classe de
              probl\`emes de {D}irichlet non lin\'{e}aires},
   JOURNAL = {Rev. Fran\c{c}aise Automat. Informat. Recherche Op\'{e}rationnelle
              S\'{e}r. Rouge Anal. Num\'{e}r.},
  FJOURNAL = {Revue Fran\c{c}aise d'Automatique, Informatique et Recherche
              Op\'{e}rationnelle S\'{e}rie Rouge. Analyse Num\'{e}rique},
    VOLUME = {9},
      YEAR = {1975},
    NUMBER = {{\rm R}-2},
     PAGES = {41--76},
      ISSN = {0397-9342},
   MRCLASS = {65N35},
  MRNUMBER = {388811},
MRREVIEWER = {J. R. Cannon},
}


@article{Pustelnik2019,
  TITLE = {{Nonlinear denoising for characterization of solid friction under low confinement pressure}},
  AUTHOR = {Colas, Jules and Pustelnik, Nelly and Oliver, 
  Cristobal and Abry, Patrice and G{\'e}minard, Jean-Christophe 
  and Vidal, Val{\'e}rie},
  JOURNAL = {{Physical Review E }},
  PUBLISHER = {{American Physical Society (APS)}},
  VOLUME = {42},
  PAGES = {91},
  YEAR = {2019},
  DOI = {10.1103/PhysRevE.100.032803},
  PDF = {https://hal.archives-ouvertes.fr/hal-02271333/file/Colas_friction_signal_revision3.pdf},
  HAL_ID = {hal-02271333},
  HAL_VERSION = {v1},
}

@article {Edelman1988,
    AUTHOR = {Edelman, Alan},
     TITLE = {Eigenvalues and condition numbers of random matrices},
   JOURNAL = {SIAM J. Matrix Anal. Appl.},
  FJOURNAL = {SIAM Journal on Matrix Analysis and Applications},
    VOLUME = {9},
      YEAR = {1988},
    NUMBER = {4},
     PAGES = {543--560},
      ISSN = {0895-4798},
   MRCLASS = {15A52 (62H10)},
  MRNUMBER = {964668},
MRREVIEWER = {D. S. Tracy},
       DOI = {10.1137/0609045},
}


@article {Bradies-Sun2017,
    AUTHOR = {Bredies, Kristian and Sun, Hongpeng},
     TITLE = {A proximal point analysis of the preconditioned alternating
              direction method of multipliers},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {173},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {878--907},
      ISSN = {0022-3239},
   MRCLASS = {65K10 (65F08 90C25)},
  MRNUMBER = {3654261},
MRREVIEWER = {Sirma Zeynep Alparslan-G\"{o}k},
       DOI = {10.1007/s10957-017-1112-5},
}

@article {Sun2019,
    AUTHOR = {Sun, Hongpeng},
     TITLE = {Analysis of fully preconditioned alternating direction method
              of multipliers with relaxation in {H}ilbert spaces},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {183},
      YEAR = {2019},
    NUMBER = {1},
     PAGES = {199--229},
      ISSN = {0022-3239},
   MRCLASS = {65K05 (65J15 90C25 90C48)},
  MRNUMBER = {3989304},
       DOI = {10.1007/s10957-019-01535-6},
}


@article {Liu2014,
    AUTHOR = {Liu, Xianming and Zhai, Deming and Zhao, Debin and Zhai,
              Guangtao and Gao, Wen},
     TITLE = {Progressive image denoising through hybrid graph {L}aplacian
              regularization: a unified framework},
   JOURNAL = {IEEE Trans. Image Process.},
  FJOURNAL = {IEEE Transactions on Image Processing},
    VOLUME = {23},
      YEAR = {2014},
    NUMBER = {4},
     PAGES = {1491--1503},
      ISSN = {1057-7149},
   MRCLASS = {94A08},
  MRNUMBER = {3191309},
       DOI = {10.1109/TIP.2014.2303638},
}

@article {Pang2017,
    AUTHOR = {Pang, Jiahao and Cheung, Gene},
     TITLE = {Graph {L}aplacian regularization for image denoising: analysis
              in the continuous domain},
   JOURNAL = {IEEE Trans. Image Process.},
  FJOURNAL = {IEEE Transactions on Image Processing},
    VOLUME = {26},
      YEAR = {2017},
    NUMBER = {4},
     PAGES = {1770--1785},
      ISSN = {1057-7149},
   MRCLASS = {94A08},
  MRNUMBER = {3623940},
       DOI = {10.1109/TIP.2017.2651400},
}

@ARTICLE{Sha2020,
author={Sha, L. and Schonfeld, D. and Wang, J.},
title={Graph Laplacian Regularization with Sparse Coding for Image Restoration and Representation},
journal={IEEE Transactions on Circuits and Systems for Video Technology},
year={2020},
volume={30},
number={7},
pages={2000-2014},
doi={10.1109/TCSVT.2019.2913411},
art_number={8700230},
}


